Fine-grained Vibration Based Sensing Using a Smartphone

Recognizing surfaces based on their vibration signatures is useful as it can enable tagging of different locations without requiring any additional hardware such as Near Field Communication (NFC) tags. However, previous vibration based surface recognition schemes either use custom hardware for creating and sensing vibration, which makes them difficult to adopt, or use inertial (IMU) sensors in commercial off-the-shelf (COTS) smartphones to sense movements produced due to vibrations, which makes them coarse-grained because of the low sampling rates of IMU sensors. The mainstream COTS smartphones based schemes are also susceptible to inherent hardware based irregularities in vibration mechanism of the smartphones. Moreover, the existing schemes that use microphones to sense vibration are prone to short-term and constant background noises (e.g. intermittent talking, exhaust fan, etc.) because microphones not only capture the sounds created by vibration but also other interfering sounds present in the environment. In this paper, we propose VibroTag, a robust and practical vibration based sensing scheme that works with smartphones with different hardware, can extract fine-grained vibration signatures of different surfaces, and is robust to environmental noise and hardware based irregularities. We implemented VibroTag on two different Android phones and evaluated in multiple different environments where we collected data from 4 individuals for 5 to 20 consecutive days. Our results show that VibroTag achieves an average accuracy of 86.55% while recognizing 24 different locations/surfaces, even when some of those surfaces were made of similar material. VibroTag's accuracy is 37% higher than the average accuracy of 49.25% achieved by one of the state-of-the-art IMUs based schemes, which we implemented for comparison with VibroTag.

==> KamranTMC/discussion.tex <==
\presec
\section{Discussions}
\postsec
\textcolor{red}{The purpose of VibroTag is to provide a novel way of accurately recognizing surfaces using vibration sensing.
%
With the realization of this functionality, we believe
many advanced applications can be realized. 
%
Most participants in our usability study agree with the scenarios we considered,
and they also provide other possible uses of VibroTag.
}

\presub
\subsection{Potential Applications}
\postsub

These applications can be classified
into two categories based on the resulting benefits: 1) helping
users remember things, and 2) saving time for users in finding
and launching desired applications.

Applications. Hand-vs-Pocket detection, FindMyPhone (phone in car, beep no sound, me vibrate), Object Detection (Radar Cat paper), HowMuchWaterInBottle, SmartNotifications, InBuildingLandmarks, Context Aware Notifications, ElderlyCare (detect whether use is wearing the device)

Issues. 

Interesting directions. E.g. if we have enough data from enough users we can come up with generic hand 

\presub
\subsection{Robustness to Noise}
\postsub

Loud music, we do not use ultrasound frequencies. 
%
Frequencies we use can easily affected.
%
Can mitigate it, because when user places phone at a location, it stays there for a while.
%
Phone can extract an average feature over time.

\presub
\subsection{Limitation of Tolerance Range}
\postsub

We are way better than EchoTag for example. 
%
But still, might not work for least restricted scenarios.
%
We can have multiple samples of a location, randomly distributed by user.
%
But we believe, as also shown in usability study results, we do not need to be that generic (least restricted).
%
Middle scenario, where user can remember a radius area, should work great.


==> KamranTMC/system.tex <==
\presec
\postsec
\section{VibroTag}
\postsec

%\subsection{System Overview}
%
VibroTag system consists of five different phases.
%
In the first phase, smartphone is vibrated for about three seconds while the surface response to the vibration is recorded simultaneously via the phone's built-in microphone.
%
Sounds produced during vibration are sampled at fixed 44.1 kHz.
%
Second, the recorded sound is analyzed in both frequency and time domains to extract robust surface/location specific vibration signatures.
%
%Once the frequency is recognized, peak detection algorithm is run on a patch of time-series, which is rms envelop of sound signal.
%
%The repetitive  patterns in time are recorded and median is taken to extract robust features. 
%
%This further improves the robustness, as we will discuss in the following sections.
%
Third, the selected locations and their corresponding signatures are recorded in the feature-location database.
%
Fourth, VibroTag uses the feature-location database to train its classifier.
%
In the testing phase, new collected vibration signature is compared with the recordings in the feature-location database using the trained classifier, which tries to identify the location.
%
Figure \ref{fig:systemoverview} shows the system overview of VibroTag.
%
Next, we discuss how we design two major functionalities of VibroTag, \ie reliable extraction of acoustic signatures due to vibrations, and accurate classification of different locations using their respective extracted vibration signatures.

\presub
\subsection{Extraction of Acoustic Signatures}
\postsub
To differentiate between different locations, we need to extract features that can uniquely and consistently represent those locations. 
%
However, we face two major challenges when trying to achieve that in VibroTag.
%
The first challenge is posed by the background noises, \eg due to exhaust fans in restrooms and short-term human speech. 
%
The second challenge is posed by the imperfections in the smartphone's hardware (\ie the microphone and the vibrator motor) affecting the audio sampling process while the smartphone vibrates. 
%
Next, we first discuss each of these challenges in detail, and then describe how we address them in VibroTag.

%\begin{figure*}[htbp]
%	%	\vspace{-0.1in}
%	\centering
%	\captionsetup{justification=centering}    
%	\captionsetup[subfigure]{aboveskip=20pt,belowskip=20pt}
%	\subfigure[Home Bed]{
%		\includegraphics[width=0.8\columnwidth]{figs/restricted-HomeBed-Restrictedpsd1}
%		\label{fig:psdexp1}}
%	\hspace{-0.23in}
%	\subfigure[Home Bed]{
%		\includegraphics[width=0.86\columnwidth]{figs/restricted-HomeBed-Restrictedrmsenvelope2-psd}
%		\label{fig:enveopestftexp1}}
%	\label{fig:psdexpsbed}
%	\vspace{-0.2in}
%	\caption{Power Spectral Density (PSD) and Short Time Fourier Transform (STFT) plots (Home Bed scenario)}
%	\vspace{-0.25in}
%\end{figure*}
%
%\begin{figure*}[htbp]
%	\subfigure[Home Living Room Sofa]{
%		{\includegraphics[width=0.8\columnwidth]{figs/restricted-HomeLivingRoomSofa-Restrictedpsd1}}
%		\label{fig:psdexp2}}
%	\hspace{-0.21in}
%	\subfigure[Home Living Room Sofa]{
%		{\includegraphics[width=0.86\columnwidth]{figs/restricted-HomeLivingRoomSofa-Restrictedrmsenvelope2-psd}}
%		\label{fig:envelopestftexp2}}
%	%	\hspace{-0.001in}
%	\label{fig:psdexpssofa}
%	\vspace{-0.2in}
%	\caption{Power Spectral Density (PSD) and Short Time Fourier Transform (STFT) plots (Home Living Room Sofa scenario)}
%	\vspace{-0.15in}
%\end{figure*}

% \smallskip\noindent\textbf{Reducing Impact of Background Noises.} 
\presub
%\postsub
\subsubsection{Challenge 1: Impact of Background Noises}
\postsub
In the following, we use an example to show why mainstream feature extraction techniques, such as Fast Fourier Transform (FFT) based Power Spectral Density (PSD), are unsuitable for vibration based sensing on COTS smartphones when there are background noise sources present in the environment.
%
Figure \ref{fig:noise1}-\ref{fig:noise3} show FFT coefficients for both lower and higher frequency ranges corresponding to experiments conducted at the same locations on a wooden chair's cushion for (a) no noise, (b) intermittent human speech and (c) clapping scenarios.
%
We can see that the FFT features are significantly affected by these noise sources, and the frequencies produced by these noise sources are directly interfering with the frequency bands of interest for vibration based sensing.
%

%
%We want our scheme to be robust to intermittent speech, even if can not be very robust against string noise \eg music.
%
%Figures \textcolor{red}{[ADD FIGURES]} show effect of music as we increase sound on the FFT and spectrogram.
%
%We can easily see that FFT is prone to the aforementioned two types of noises.
%
To reduce the impact of such background noises in VibroTag, we take a two pronged approach. 
%
First, to remove static background noises, we take \textit{first order differential} of the \textit{root mean squared} (RMS) envelope of the recorded sound signals.
%
We choose RMS envelope for our analysis as it gives us a measure of the power of the vibration signal, while producing a waveform that is easy to analyze. 
%
Moreover, short-term and higher frequency noisy variations are averaged out in the envelope signal, while it still keeps most of the useful vibration response related information intact.
%
We take RMS envelope of the signal over a sliding window of N samples, where N = 15 audio samples in our current implementation of VibroTag.
%
%This phenomenon will soon be evident in what follows.
%
\textit{From now onward, when we mention the term \textit{audio/sound signal}, we mean the first order difference of the RMS envelope of that audio/sound signal}.
%
Second, to reduce impact of short-term noises (similar to Figs. \ref{fig:noise2}-\ref{fig:noise3}), we vibrate the phone for at least 3 seconds for every experiment, and then extract multiple vibration patterns across time that we combine in the end to get a single consistent vibration signature.
%
We will discuss how we extract such signatures in \S \ref{sec:timeseries}.
%
Figure \ref{fig:noise4} shows the signatures extracted by VibroTag for the experiments corresponding to Figs. \ref{fig:noise1}-\ref{fig:noise3}, which are consistent and almost identical.
%
%\textcolor{red}{We also allow frequencies between 20 - 5500 Hz only, which is human hearing range, just to remove any unwanted noises in higher frequencies.}

\begin{figure*}[htbp]
	%	\vspace{-0.1in}
	\centering
	\captionsetup{justification=centering}    
	\captionsetup[subfigure]{aboveskip=-1pt,belowskip=-1pt}
	\subfigure[Home Bed]{
		\includegraphics[width=1.042\columnwidth]{figs/restricted-HomeBed-Restricteddetectedpeaks5}
		\label{fig:peaksexp1}}
	\hspace{-0.22in}
	\subfigure[Home Living Room Sofa]{
		{\includegraphics[width=1.042\columnwidth]{figs/restricted-HomeLivingRoomSofa-Restricteddetectedpeaks5}}
		\label{fig:peaksexp2}}
	%	\hspace{-0.001in}
	\label{fig:peaksexps}
	\vspace{-0.15in}
	\caption{Repetitive patterns appearing in the processed sound signals corresponding to vibration}
	\vspace{-0.22in}
\end{figure*}

%\smallskip\noindent\textbf{Dealing with Hardware Imperfections.} 
\presub
\postsub
\subsubsection{Challenge 2: Hardware Imperfections}
\postsub
In the following, we use some examples to show why mainstream feature extraction techniques, such as PSD as well as Short Time Fourier Transform (STFT), are unsuitable for vibration based sensing on COTS smartphones when there are irregularities in the vibration sensing process due to hardware imperfections.
%
Figures \ref{fig:psdexp1} and \ref{fig:psdexp2} show the PSD of the recorded/unprocessed sound signals for multiple different experiments which we performed by placing a smartphone at the same location on a sofa and a bed, respectively.
%
Each figure shows the PSD coefficients over two different frequency ranges.
%
We can observe that PSDs for both the sofa and the bed are not consistent for repetitive experiments, even when the smartphone's location and the environmental scenario while performing the experiments remained unchanged.
%
This occurs because the smartphone, its vibrator motor, and the rest of its hardware vibrate at slightly different frequencies in each different experiment.
%
This behavior is random and uncontrollable, and therefore, is bound to cause intra-class (\ie within samples of the same class) variations which will lead to classification errors.
%
Moreover, Figs. \ref{fig:psdexp1} and \ref{fig:psdexp2} show that some experiments corresponding to the two different surfaces show variations in the same set of frequencies, which further makes usage of such frequency domain features infeasible as they cannot be used to uniquely represent different surfaces.
%

%
Analyzing the audio signals in just frequency domain also leads to complete loss of time domain information.
%
Therefore, to take a look into variations caused by smartphone vibrations across both frequency and time domains, we leverage STFT or \textit{spectrogram}.
%
Figures \ref{fig:enveopestftexp1} and \ref{fig:envelopestftexp2} show STFT of the recorded audio signals corresponding to the same two aforementioned scenarios.
%
We observe that the STFTs of both surfaces are very similar, and often occur in the same frequency ranges that makes it harder to differentiate between those surfaces.
%
Interestingly, we also notice some patterns repeating along time; however, the time period of their repetition is not consistent.
%
As we discussed in \S \ref{sec:workingprinciples}, smartphone vibrations are generated because of the to and fro motion of a mass inside its vibration motor.
%
The vibration motor tries to move the smartphone (and the hardware inside) at its own vibration frequency (which is often irregular due hardware imperfections).
%
However, the smartphone's motion is constrained due to its own weight/structure, and because of the absorption properties of the surface it is placed on.
%
This whole process during vibration gives rise to peculiar pressure waves, which are sensed by the built-in microphone.
%
Moreover, as the mass inside the vibrator motor repeatedly moves to and fro, it will give rise to similar pressure waves every cycle of its ``irregular'' vibration period, which will reflect in time-series of the sound signals.
%
Therefore, we hypothesize that even if there are irregularities in the repetition frequency of such patterns, the patterns themselves must be very similar.
%
This intuition forms the basis of our time-series based analysis of the surfaces' vibration response, which we present next.

%\begin{figure}[htbp]
%	%	\vspace{-0.1in}
%	\centering
%	\captionsetup{justification=centering}    
%	\captionsetup[subfigure]{aboveskip=-1pt,belowskip=-1pt}
%	\subfigure[Home Bed]{
%		\includegraphics[width=0.75\columnwidth]{figs/restricted-HomeBed-Restrictedrmsenvelope2-psd}
%		\label{fig:enveopestftexp1}}
%	%	\hspace{-0.1in}
%	\subfigure[Home Living Room Sofa]{
%		{\includegraphics[width=0.75\columnwidth]{figs/restricted-HomeLivingRoomSofa-Restrictedrmsenvelope2-psd}}
%		\label{fig:envelopestftexp2}}
%	%	\hspace{-0.001in}
%	\label{fig:enveopestftexp}
%	\vspace{-0.2in}
%	\caption{Short Time Fourier Transform (STFT) examples}
%	\vspace{-0.15in}
%\end{figure}

\vspace{-0.03in}
\presub
\subsubsection{Time-Series Analysis of Vibration Response} \label{sec:timeseries}
\postsub
In the following, we discuss our time-series based analysis of the processed sound signals corresponding to vibration.
%
Figures \ref{fig:peaksexp1} and \ref{fig:peaksexp2} show time-series of the processed sound signals (\ie first order difference of the RMS envelope) corresponding to one of the experiments from each of the two different surfaces (\ie the Bed and the Sofa) whose FFT's were shown in \ref{fig:psdexp1} and \ref{fig:psdexp2}, respectively.
%
The two time-series correspond to a window of 4800 audio samples (\ie $\sim$0.1088 seconds).
%
We can evidently see peculiar patterns repeating in both time-series, which repeat approximately with the frequency of vibrating mass in the smartphone's vibration motor.
%
We also observe that the time-series patterns in both scenarios are consistent across time, and that the patterns in one scenario is different from the ones in other.
%
This difference was not observable in the previous frequency based analyses.
%
Our aim is to use these patterns as features to robustly differentiate surfaces.
%
However, two challenges arise: \textit{(1) How can we correctly extract these features, given that the frequency of their repetition and place of their occurrence is not exactly known?}, and (2) \textit{How do we make sure that features we extract over a certain time window also repeat in other time windows, and therefore, truly represent the surface's vibration response?}
%
To answer these questions, we employ a peak detection based scheme to detect the time-series patterns which occur over time during vibration, and then take median of all the extracted patterns to get a single consistent vibration signature.
%
Next, we present our vibration signature extraction algorithm.

\presub
\postsub
\subsubsection{Time-Series Signature Extraction Algorithm}
\postsub
VibroTag extracts vibration signature from the processed sound signals in four steps: (1) Randomly select different time-series windows, each of size S (S=4800 samples in our current implementation), then for each time window, (2) perform \textit{max-min normalization} on the whole time-series in the selected window, (3) perform FFT analysis to extract the frequency corresponding to highest amplitude (which will correspond to the approximate repetition frequency of the time-series patterns), (4) identify the patterns by detecting peaks, (5) extract the time-series patterns between consecutive peaks, (6) check if at least M valid features have been extracted over different time windows (M=100 in our implementation), and then finally, (7) combine all the extracted patterns from all the time windows by taking their median.
%
Next, we explain steps (2)-(7).

Once a time window is randomly selected, in the second step, VibroTag max-min normalizes the whole time-series in the selected window. 
%
This step ensures that the parametrization of our peak detection algorithm can be easily generalized.
%
As we discussed before, the frequency of repetition ($f_o$) of vibration patterns in the processed sound signal is irregular.
%
However, peak detection based feature extraction approach requires an approximate number for $f_o$ (\ie $\hat{f}_{o}$) to work effectively and robustly.
%
Therefore, in the third step, VibroTag calculates PSD of the signal in the selected window.
%
Figures \ref{fig:envelopermspsd1} and \ref{fig:envelopermspsd2} show example PSD's corresponding to seven different experiments performed on the Bed and the Sofa, respectively.
%
Based on the PSD, VibroTag determines the peak frequency which corresponds to the approximate repetition frequency (\ie $\hat{f}_{o}$) of the vibration patterns.
%
This value is then used by our peak detection algorithm, which is the fourth step.
%
\begin{figure}[htbp]
%	\vspace{-0.13in}
	\centering
	\captionsetup{justification=centering}    
	\captionsetup[subfigure]{aboveskip=20pt,belowskip=20pt}
	\subfigure[Home Bed]{
		\includegraphics[width=0.49\columnwidth]{figs/restricted-HomeBed-Restrictedpsd2}
		\label{fig:envelopermspsd1}}
	\hspace{-0.21in}
	\subfigure[Home Living Room Sofa]{
		{\includegraphics[width=0.49\columnwidth]{figs/restricted-HomeLivingRoomSofa-Restrictedpsd2}}
		\label{fig:envelopermspsd2}}
	%	\hspace{-0.001in}
	\label{fig:envelopermspsd}
	\vspace{-0.15in}
	\caption{PSD of the sound signals in time windows corresponding to the scenarios in Figs. \ref{fig:peaksexp1}-\ref{fig:peaksexp2}}
	\vspace{-0.13in}
\end{figure}

In the fourth step, VibroTag's peak detection algorithm detects vibrations patterns in the selected window based on three key parameters, namely \textit{minimum peak prominence} (MINPRO), \textit{minimum peak distance} (MINDIST), and \textit{minimum peak strength} (MINSTR), to robustly detect the number of peaks.
%
The prominence of a peak measures how much the peak stands out, due to its height and location, relative to other peaks around it. 
%
We tune MINPRO such that we only detect those peaks which have a relative importance of at least MINPRO.
%
We tune MINDIST according to the fact that maximum repetition rate of patterns is approximately $\hat{f}_{o} + \delta f$, such that the redundant peaks are discarded. 
%
We set $\delta f$ as the second standard deviation of the variation in vibration frequency around $\hat{f}_{o}$, which we estimate using multiple different experiments.
%
$\delta f$ is required as some vibration patterns can repeat earlier than $1/\hat{f}_{o}$.
%
To further sift out redundant peaks, we only choose peaks of value greater than MINSTR times the median peak value in the selected time window.
%
In our current implementation, we chose MINPRO = 0.65, MINDIST = $\frac{1}{f_o + \delta f}$ seconds, $\delta f = 6.5$,  and MINSTR = 0.5.
%
We perform this parametrization only during the design of our system, which generalizes well for multiple different surfaces and smartphones (\ie Nexus 4 and OnePlus 2).
%
VibroTag does not require end-user calibration effort in real-world deployments.

In the fifth step, VibroTag uses the consecutive peaks detected in each randomly selected window to extract multiple vibration patterns between those peaks.
%
In the sixth step, VibroTag checks if at least a total of $M=100$ patterns have been extracted from all the time windows. 
%
If VibroTag is not able to find peaks and extract valid vibration patterns in a window, it keeps randomly selecting new windows, and the process is repeated until $M=100$ patterns are extracted.
%
\textit{In real-life scenarios, the number of iterations required to extract $M$ vibration patterns of a surface can be used to tell the user whether their environment is too noisy to extract a valid vibration signature or not.}
%
For example, the average (taken over 20 different samples) number of iterations it took for convergence when loud music (\ie variable noise) was played in the background was $\sim$1351, for medium noise/volume level the number was $\sim$495, whereas for no variable noise scenarios it was $\sim$136.
%


In the final step, VibroTag combines all the extracted vibration patterns using median (loses anything lying outside 75\% of data) to get a single vibration signature.
%
%Figure \textcolor{red}{ADD FIGURE} shows how noisy samples lead to higher number of iterations required for convergence of M.
%
The median operation helps VibroTag remove short-term noisy variations in different vibration patterns, and therefore, allows it to extract a single robust vibration signature of the surface.
%
Figures \ref{fig:finalfeaturesexp1} and \ref{fig:finalfeaturesexp2} show the example signatures extracted for the Bed and the Sofa related experiments, where we can observe that the vibration signatures of each surface are consistent and almost identical.
%
Moreover, the extracted signatures uniquely represent their respective surfaces.
%
\begin{figure}[htbp]
	\vspace{-0.1in}
	\centering
	\captionsetup{justification=centering}    
	\captionsetup[subfigure]{aboveskip=-1pt,belowskip=-1pt}
	\subfigure[Home Bed]{
		\includegraphics[width=0.48\columnwidth,height=0.31\columnwidth]{figs/restricted-HomeBed-RestrictedFeatures}
		\label{fig:finalfeaturesexp1}}
	\hspace{-0.15in}
	\subfigure[Home Living Room Sofa]{
		{\includegraphics[width=0.48\columnwidth,height=0.31\columnwidth]{figs/restricted-HomeLivingRoomSofa-RestrictedFeatures}}
		\label{fig:finalfeaturesexp2}}
%	\subfigure[Cafeteria Table 1]{
%		{\includegraphics[width=0.48\columnwidth,height=0.32\columnwidth]{figs/implementation/cafe-table1-feature}}
%		\label{fig:cafetable1}}
%	\hspace{-0.15in}
%	\subfigure[Cafeteria Table 2]{
%		{\includegraphics[width=0.47\columnwidth,height=0.32\columnwidth]{figs/implementation/cafe-table2-feature}}
%		\label{fig:cafetable2}}
%	\subfigure[DTW Distance Matrix]{
%			\includegraphics[width=0.7\columnwidth]{figs/restricted-HomeLivingRoomSofa-HomeBed-RestrictedDTW}
%		\label{fig:restricted-homelivingroomsofa-homebed-restricteddtw}
%	}
	%	\hspace{-0.001in}
	\label{fig:finalfeaturesexps}
	\vspace{-0.15in}
	\caption{Extracted time-series features (Low Noise)}
	\vspace{-0.13in}
\end{figure}

Figures \ref{fig:cafetablesnoise} show the example signatures extracted for two different tables during lunch time in a cafeteria on university campus (\ie very noisy environment). 
%
We can see that although some vibration signatures are noisy, yet VibroTag is able to extract consistent vibration signatures in highly noisy environments as well.

\begin{figure}[htbp]
	\vspace{-0.1in}
	\centering
	\captionsetup{justification=centering}
	\subfigure[Cafeteria Table 1]{
		{\includegraphics[width=0.48\columnwidth,height=0.31\columnwidth]{figs/implementation/cafe-table1-feature}}
		\label{fig:cafetable1}}
	\hspace{-0.15in}
	\subfigure[Cafeteria Table 2]{
		{\includegraphics[width=0.47\columnwidth,height=0.31\columnwidth]{figs/implementation/cafe-table2-feature}}
		\label{fig:cafetable2}}
	\hspace{-0.1in}
	\vspace{-0.13in}
	\caption{Extracted time-series features (High Noise)}
	\centering
	\vspace{-0.13in}
	\label{fig:cafetablesnoise}
\end{figure}

\presub
\subsection{Classification Training}
\postsub
%We use these shapes of the extracted waveforms as features because the shapes retain both time and frequency domain information of the waveforms and are thus more suited for use in classification.
%
After obtaining the time-series vibration signatures, VibroTag uses them to build training models for classification.
%
As VibroTag needs to compare vibration signatures obtained for different surfaces, we need a comparison metric that provides an effective measure of similarity between vibration signatures of two surfaces.
%
To achieve this, VibroTag uses a well-known method called Dynamic Time Warping (DTW) that calculates the distance between waveforms by performing optimal alignment between them. 
%
Using DTW distance as the comparison metric between vibration signatures, VibroTag trains a k-nearest neighbour (kNN) classifier using those signatures. 
%
Next, we first explain how we apply DTW on the vibration signatures, and then explain how we train
the kNN classifier.

\begin{figure}
%	\vspace{-0.1in}
	\centering
	\captionsetup{justification=centering}
	\includegraphics[width=0.7\columnwidth]{figs/restricted-HomeLivingRoomSofa-HomeBed-RestrictedDTW}
	\vspace{-0.1in}
	\caption{DTW Distance Matrix (First 12 = Bed scenario, Second 12 = Living Room Sofa scenario)}
	\vspace{-0.2in}
	\label{fig:restricted-homelivingroomsofa-homebed-restricteddtw}
\end{figure}

\presub
\subsubsection{Dynamic Time Warping}
\postsub
DTW is a dynamic programming based solution for obtaining
minimum distance alignment between any two waveforms.
%
DTW can handle waveforms of different lengths and
allows a non-linear mapping of one waveform to another by
minimizing the distance between the two. 
%
In contrast to Euclidean distance, DTW gives us intuitive distance between
two waveforms by determining minimum distance warping
path between them even if they are distorted or shifted
versions of each other. 
%
DTW distance is the Euclidean distance
of the optimal warping path between two waveforms
calculated under boundary conditions and local path constraints
\textcolor{red}{[25]}. 
%
In our experiments, DTW distance proves to
be very effective metric for comparing two vibration signatures of
different surfaces.
%
%\textcolor{red}{VibroTag uses local path constraints of 27, 45, and
%63 degrees while determining minimum cost warping path
%between two waveforms.}
%
For the vibration signatures extracted from the experiments corresponding to the bed and the sofa (shown in Fig.~\ref{fig:restricted-homelivingroomsofa-homebed-restricteddtw}), the average DTW distance among signatures of the Bed was $\sim$2.3 and the DTW distance among signatures of the Sofa was $\sim$3.1.
%
However, the average DTW distance between the vibration signatures of these surfaces was 16.59.

\presub
\subsubsection{Classifier Training}
\postsub
%To maximize the advantage of having multiple shape features per keystroke obtained from multiple transmit-receive antenna pairs, we build separate classifiers for each of those
%shape features. 
%
%\textcolor{red}{Also write how k = 5 works, why neighbors needed and why they can help if our guy matches with an outlier from the other class.}
%
VibroTag requires the user to provide training data for the surfaces to be recognized.
%
Afterwards, it trains a kNN classifier using the vibration signatures corresponding to those surfaces. 
%
To recognize a surface, VibroTag feeds the detected vibration feature of that surface to the trained kNN classifier. 
%
The kNN classifier searches for the majority class label among k nearest neighbors of the corresponding vibration signature using DTW distance metric.
%
VibroTag declares the majority class label obtained from the kNN classifier as label of the tested surface.
%
In the current implementation of VibroTag, we chose k = 5 so that the classification process averages more voters in each prediction and hence is more resilient to outliers.


==> biography.tex <==
\begin{IEEEbiography}
%
[{\includegraphics[width=1in,height=1.10in,clip,keepaspectratio]{figs/kamran}}]{Kamran Ali}
%
is a Ph.D. candidate at Department of Computer Science and Engineering, Michigan State University, USA.
%
He received his B.S. degree in Electrical Engineering and Computer Sciences in 2013, from School of Science and Engineering (SSE) of Lahore University of Management
Sciences (LUMS), Pakistan.
%
He has worked with Hewlett Packard Labs, NEC Laboratories, Nokia Bell Labs and Microsoft's Applied Sciences Group. 
%
His research interests lie in the areas of Sensing Systems, Applied Machine Learning, Wireless Communications, RF Sensing, Mobile Computing, Pervasive Computing, Signal Processing, and Internet of Things.
%
\end{IEEEbiography}
%
\vspace{-0.5in}
%
\begin{IEEEbiography}
%
[{\includegraphics[width=1in,height=1.10in,clip,keepaspectratio]{figs/alex}}]{Alex X. Liu}
received his Ph.D. degree in Computer Science from The University of Texas at Austin in 2006, and is a professor at the Department of Computer Science and Engineering, Michigan State University. He received the IEEE \& IFIP William C. Carter Award in 2004, a National Science Foundation CAREER award in 2009, and the Michigan State University Withrow Distinguished Scholar Award in 2011. He has served as an Editor for IEEE/ACM Transactions on Networking, and he is currently an Associate Editor for IEEE Transactions on Dependable and Secure Computing and IEEE Transactions on Mobile Computing, and an Area Editor for Computer Communications. He has served as the TPC Co-Chair for ICNP 2014 and IFIP Networking 2019. He received Best Paper Awards from ICNP-2012, SRDS-2012, and LISA-2010. His research interests focus on networking and security. He is a Fellow of the IEEE.
%
\end{IEEEbiography}
